TinyTurbo: Efficient Turbo Decoders on Edge

In this paper, we introduce a neural-augmented decoder for Turbo codes called TINYTURBO . TINYTURBO has complexity comparable to the classical max-log-MAP algorithm but has much better reliability than the max-log-MAP baseline and performs close to the MAP algorithm. We show that TINYTURBO exhibits strong robustness on a variety of practical channels of interest, such as EPA and EVA channels, which are included in the LTE standards. We also show that TINYTURBO strongly generalizes across different rate, blocklengths, and trellises. We verify the reliability and efficiency of TINYTURBO via over-the-air experiments.

==> conclusion.tex <==
% !TEX root = main.tex

%\section{Conclusion}

==> results_old.tex <==
% !TEX root = main.tex

\section{Results}

Figure 1: Turbo(40,132) AWGN Channels.  
Figure 2: 



%---------------- 

\subsection{AWGN channel}

% Short blocklength
\begin{figure}[htbp]
  \centering
  \includegraphics[width=0.3\textwidth]{new_figures/new_bl40_awgn.pdf}
    \put(-125,32){\fontsize{3}{5}\selectfont Max-log-MAP 3 iters}
    \put(-125,27){\fontsize{3}{5}\selectfont MAP 6 iters}
    \put(-125,22){\fontsize{3}{5}\selectfont Turbonet+ \cite{he2020modeldriven}}
    \put(-125,17){\fontsize{3}{5}\selectfont TinyTurbo}
    \put(-125,0){\footnotesize Signal-to-noise ratio (SNR) [dB]}
    \put(-155,53){\rotatebox[origin=t]{90}{\footnotesize Error rate}}
  \caption{Turbo(40,132) , AWGN test: TinyTurbo (3 iter)  outperforms TurboNet+ even if it has much less parameters (18 as opposed to 40*3*6). TinyTurbo 3 iterations is comparable to MAP 6 iterations.}
  \label{fig:bl40_awgn} 
    %  \vspace{-0.08in}
\end{figure}




\iffalse
    { \todo Naming: MAP - 6 iterations, Max-log-MAP - 3 iterations (or 6?) TinyTurbo - 3 iterations, TurboNet+ [Reference] }
    
        - Entangling the weights does not hurt. 
    
        % Robustness   within AWGN   
        - Different blocklengths (40,~100, {\todo ~1000}). Hope is that for longer blocklengths we save a lot of parameters with faster convergence and better performance.
        % diff code (757) and rate 
        - Rate 1/3 - different block lengths. Rate 1/2 (with puncturing). (40, 100, 1000) block lengths.  
        
        % LLR vs Raw bit training 
        - Raw bit training vs. LLR Training - different channels robustness, etc? 
        
        - Training time: Convergence curves. Blocklengths 100 and 1000. 
        
        - TurboNet+ with entangled weights. Gains coming from our loss function.
\fi 



\subsection{Robustness across channels}


\begin{figure}[htbp]
  \centering
  \includegraphics[width=0.3\textwidth]{new_figures/bl40_bursty.pdf}
    \put(-125,32){\fontsize{3}{5}\selectfont Max-log-MAP 3 iters}
    \put(-125,27){\fontsize{3}{5}\selectfont MAP 6 iters}
    \put(-125,22){\fontsize{3}{5}\selectfont Turbonet+ \cite{he2020modeldriven}}
    \put(-125,17){\fontsize{3}{5}\selectfont TinyTurbo}
    \put(-125,0){\footnotesize Signal-to-noise ratio (SNR) [dB]}
    \put(-155,53){\rotatebox[origin=t]{90}{\footnotesize Error rate}}
  \caption{Turbo(40,132) , Bursty channel test}
  \label{fig:bl40_bursty}
    %  \vspace{-0.08in}

\end{figure}

\subsection{Adaptivity}


\begin{figure}[htbp]
  \centering
  \includegraphics[width=0.3\textwidth]{new_figures/bl40_bursty_retrained.pdf}
    \put(-125,37){\fontsize{3}{5}\selectfont Max-log-MAP 3 iters}
    \put(-125,32){\fontsize{3}{5}\selectfont MAP 6 iters}
    \put(-125,27){\fontsize{3}{5}\selectfont Turbonet+}
    \put(-125,22){\fontsize{3}{5}\selectfont TinyTurbo - AWGN trained \cite{he2020modeldriven}}
    \put(-125,17){\fontsize{3}{5}\selectfont TinyTurbo - Bursty retrained}
    \put(-125,0){\footnotesize Signal-to-noise ratio (SNR) [dB]}
    \put(-155,53){\rotatebox[origin=t]{90}{\footnotesize Error rate}}
  \caption{Turbo(40,132) , Retrained on bursty channel}
  \label{fig:bl40_bursty_retrain}
    %  \vspace{-0.08in}

\end{figure}


\iffalse
    \subsection{Robustness and adaptivity}
    
        - Robustness across channels (Standard channels and OTA) 
        
        - Adaptivity (Standard channels and OTA) 
    
    
        Channel models: Bursty (show until hitting the error floor), EPA, EVA (increase the SNR BER hitting $10^{-5}$), OTA-1 (static, indoor), OTA-2 (some time-varying obstacles/nodes).
        
        \todo Share weights with Rajesh. He will plot on MATLAB for EPA, EVA. 
        
        - \todo Robustness with respect to block lengths: Plot Ours, Max-log-MAP, MAP all with 3 iterations and 6 iterations.
    
\fi 

\subsection{On device implementation}
    On-device aspect? inference latency "measurement" difference between two time stamps (processing on the chip) 



    
    
\subsection{Interpretability}




%%%%%%
%% An example of a floating figure using the graphicx package.
%% Note that \label must occur AFTER (or within) \caption.
%% For figures, \caption should occur after the \includegraphics.
%%

%%%%%%
%% Sample figure
%%%%%%


% \begin{figure}[h]
%     \centering
% \includegraphics[width=.4\textwidth]{Plots_for_paper/results_92.pdf}
%     \put(-157,35){\fontsize{4}{5}\selectfont RM(9,2) BLER}
%     \put(-157,30){\fontsize{4}{5}\selectfont \KO(9,2) BLER}
%     \put(-157,25){\fontsize{4}{5}\selectfont RM(9,2) BER}
%     \put(-157,20){\fontsize{4}{5}\selectfont \KO(9,2) BER}
%     \put(-153,0){\footnotesize Signal-to-noise ratio (SNR) [dB]}
%     \put(-192,63){\rotatebox[origin=t]{90}{\footnotesize Error rate}}
%     % \vspace{-0.1cm}
%     \caption{ $\KO(9,2)$, discovered by training a neural network with a carefully chosen architecture in \S\ref{sec:neural_ko}, significantly improves upon state-of-the-art RM$(9,2)$ both in BER and BLER. (For both codes, the code block length is $2^9 = 512$ and the number of transmitted message bits is ${9 \choose 0}+{9 \choose 1}+{9 \choose 2} = 55$. Also, both codes are decoded using successive cancellation decoding with similar decoding complexity)}
%     \label{fig:1} 
%     %  \vspace{-0.08in}
% \end{figure}



% \begin{figure}[htbp]
%   \centering
%   \includegraphics[width=0.3\textwidth]{figures/bl40_awgn.png}
%   % where an .eps filename suffix will be assumed under latex,
%   % and a .pdf suffix will be assumed for pdflatex
%   \caption{Turbo(40,132) , AWGN test}
%   \label{fig:bl40_awgn}
% \end{figure}



% \begin{figure}[htbp]
%   \centering
%   \includegraphics[width=0.3\textwidth]{figures/bl40_logmap_train.png}
%   % where an .eps filename suffix will be assumed under latex,
%   % and a .pdf suffix will be assumed for pdflatex
%   \caption{Turbo(40,132) , Trained with Log-MAP BCJR}
%   \label{fig:bl40_logmap}
% \end{figure}

\begin{figure}[htbp]
  \centering
  \includegraphics[width=0.3\textwidth]{new_figures/new_bl40_logmap_train.pdf}
    \put(-125,37){\fontsize{3}{5}\selectfont Max-log-MAP 3 iters}
    \put(-125,32){\fontsize{3}{5}\selectfont MAP 3 iters}
    \put(-125,27){\fontsize{3}{5}\selectfont MAP 6 iters}
    \put(-125,22){\fontsize{3}{5}\selectfont Turbonet+ \cite{he2020modeldriven}}
    \put(-125,17){\fontsize{3}{5}\selectfont TinyTurbo}
    \put(-125,0){\footnotesize Signal-to-noise ratio (SNR) [dB]}
    \put(-155,53){\rotatebox[origin=t]{90}{\footnotesize Error rate}}
  \caption{Turbo(40,132) , Trained with MAP BCJR}
  \label{fig:bl40_map}
    %  \vspace{-0.08in}

\end{figure}

% \begin{figure}[htbp]
%   \centering
%   \includegraphics[width=0.3\textwidth]{figures/bl40_bursty.png}
%   % where an .eps filename suffix will be assumed under latex,
%   % and a .pdf suffix will be assumed for pdflatex
%   \caption{Turbo(40,132) , Bursty channel test}
%   \label{fig:bl40_bursty}
% \end{figure}


% \begin{figure}[htbp]
%   \centering
%   \includegraphics[width=0.3\textwidth]{figures/bl40_bursty_retrained.png}
%   % where an .eps filename suffix will be assumed under latex,
%   % and a .pdf suffix will be assumed for pdflatex
%   \caption{Turbo(40,132) , Bursty channel adaptivity}
%   \label{fig:bl40_bursty_adaptivity}
% \end{figure}

% \begin{figure}[htbp]
%   \centering
%   \includegraphics[width=0.3\textwidth]{figures/bl40_epa.png}
%   % where an .eps filename suffix will be assumed under latex,
%   % and a .pdf suffix will be assumed for pdflatex
%   \caption{Turbo(40,132) , EPA channel test}
%   \label{fig:bl40_epa}
% \end{figure}

% \begin{figure}[htbp]
%   \centering
%   \includegraphics[width=0.3\textwidth]{figures/bl40_eva.png}
%   % where an .eps filename suffix will be assumed under latex,
%   % and a .pdf suffix will be assumed for pdflatex
%   \caption{Turbo(40,132) , EVA channel test}
%   \label{fig:bl40_eva}
% \end{figure}

% \begin{figure}[htbp]
%   \centering
%   \includegraphics[width=0.3\textwidth]{figures/bl104_awgn.png}
%   % where an .eps filename suffix will be assumed under latex,
%   % and a .pdf suffix will be assumed for pdflatex
%   \caption{Turbo (104,324) , AWGN test}
%   \label{fig:bl104_awgn}
% \end{figure}

% \begin{figure}[htbp]
%   \centering
%   \includegraphics[width=0.3\textwidth]{figures/bl104_bursty.png}
%   % where an .eps filename suffix will be assumed under latex,
%   % and a .pdf suffix will be assumed for pdflatex
%   \caption{Turbo(104,324) , Bursty channel test}
%   \label{fig:bl104_bursty}
% \end{figure}

\begin{figure}[htbp]
  \centering
  \includegraphics[width=0.3\textwidth]{new_figures/bl104_bursty.pdf}
    \put(-125,32){\fontsize{3}{5}\selectfont Max-log-MAP 3 iters}
    \put(-125,27){\fontsize{3}{5}\selectfont MAP 6 iters}
    \put(-125,22){\fontsize{3}{5}\selectfont Turbonet+ \cite{he2020modeldriven}}
    \put(-125,17){\fontsize{3}{5}\selectfont TinyTurbo}
    \put(-125,0){\footnotesize Signal-to-noise ratio (SNR) [dB]}
    \put(-155,53){\rotatebox[origin=t]{90}{\footnotesize Error rate}}
  \caption{Turbo(104,324) , Bursty channel test}
  \label{fig:bl104_bursty}
    %  \vspace{-0.08in}

\end{figure}

\begin{figure}[htbp]
  \centering
  \includegraphics[width=0.3\textwidth]{new_figures/bl104_bursty_retrained.pdf}
    \put(-125,37){\fontsize{3}{5}\selectfont Max-log-MAP 3 iters}
    \put(-125,32){\fontsize{3}{5}\selectfont MAP 6 iters}
    \put(-125,27){\fontsize{3}{5}\selectfont Turbonet+}
    \put(-125,22){\fontsize{3}{5}\selectfont TinyTurbo - AWGN trained \cite{he2020modeldriven}}
    \put(-125,17){\fontsize{3}{5}\selectfont TinyTurbo - Bursty retrained}
    \put(-125,0){\footnotesize Signal-to-noise ratio (SNR) [dB]}
    \put(-155,53){\rotatebox[origin=t]{90}{\footnotesize Error rate}}
  \caption{Turbo(104,324) , Retrained on bursty channel}
  \label{fig:bl104_bursty_retrain}
    %  \vspace{-0.08in}

\end{figure}

% \begin{figure}[htbp]
%   \centering
%   \includegraphics[width=0.3\textwidth]{figures/bl104_bursty_retrained.png}
%   % where an .eps filename suffix will be assumed under latex,
%   % and a .pdf suffix will be assumed for pdflatex
%   \caption{Turbo(104,324) , Bursty channel adaptivity}
%   \label{fig:bl104_bursty_adaptivity}
% \end{figure}

% \begin{figure}[htbp]
%   \centering
%   \includegraphics[width=0.3\textwidth]{figures/bl104_epa.png}
%   % where an .eps filename suffix will be assumed under latex,
%   % and a .pdf suffix will be assumed for pdflatex
%   \caption{Turbo(104,324) , EPA channel test}
%   \label{fig:bl104_epa}
% \end{figure}

% \begin{figure}[htbp]
%   \centering
%   \includegraphics[width=0.3\textwidth]{figures/bl104_eva.png}
%   % where an .eps filename suffix will be assumed under latex,
%   % and a .pdf suffix will be assumed for pdflatex
%   \caption{Turbo(104,324) , EVA channel test}
%   \label{fig:bl104_eva}
% \end{figure}

\begin{figure}[htbp]
  \centering
  \includegraphics[width=0.3\textwidth]{new_figures/new_bl40_punctured.pdf}
    \put(-125,32){\fontsize{3}{5}\selectfont Max-log-MAP 3 iters}
    \put(-125,27){\fontsize{3}{5}\selectfont MAP 6 iters}
    \put(-125,22){\fontsize{3}{5}\selectfont Turbonet+ \cite{he2020modeldriven}}
    \put(-125,17){\fontsize{3}{5}\selectfont TinyTurbo}
    \put(-125,0){\footnotesize Signal-to-noise ratio (SNR) [dB]}
    \put(-155,53){\rotatebox[origin=t]{90}{\footnotesize Error rate}}
  \caption{Turbo(40,92) - punctured , AWGN test}
  \label{fig:bl40_punc}
    %  \vspace{-0.08in}

\end{figure}

\begin{figure}[htbp]
  \centering
  \includegraphics[width=0.3\textwidth]{figures/ota_robustness.png}
  % where an .eps filename suffix will be assumed under latex,
  % and a .pdf suffix will be assumed for pdflatex
  \caption{Turbo(40,132) , OTA robustness}
  \label{fig:bl40_ota_robustness}
\end{figure}

\begin{figure}[htbp]
  \centering
  \includegraphics[width=0.3\textwidth]{figures/ota_adaptivity.png}
  % where an .eps filename suffix will be assumed under latex,
  % and a .pdf suffix will be assumed for pdflatex
  \caption{Turbo(40,132) , OTA adaptivity}
  \label{fig:bl40_ota_adaptivity}
\end{figure}

\begin{figure}[htbp]
  \centering
  \includegraphics[width=0.3\textwidth]{new_figures/tn_training_loss.pdf}
  % where an .eps filename suffix will be assumed under latex,
  % and a .pdf suffix will be assumed for pdflatex
  \caption{Turbo(40,132) , training loss}
  \label{fig:bl40_ota_adaptivity}
\end{figure}


\begin{figure}[htbp]
  \centering
  \includegraphics[width=0.3\textwidth]{new_figures/tn_training_bers.pdf}
  % where an .eps filename suffix will be assumed under latex,
  % and a .pdf suffix will be assumed for pdflatex
  \caption{Turbo(40,132) , training BERs: TT converges faster than TT w/o weight sharing. W.r.t Turbonet+, converges to a better BER.}
  \label{fig:bl40_ota_adaptivity} % TinyTurbo with two training methodologies 
\end{figure}
%%%%%%

